Simulations of DNA-origami self-assembly reveal design-dependent nucleation barriers

Nucleation is the rate-determining step in the kinetics of many self-assembly processes. However, the importance of nucleation in the kinetics of DNA-origami self-assembly, which involves both the binding of staple strands and the folding of the scaffold strand, is unclear. Here, using Monte Carlo simulations of a lattice model of DNA origami, we find that some, but not all, designs can have a nucleation barrier and that this barrier disappears at lower temperatures, rationalizing the success of isothermal assembly. We show that the height of the nucleation barrier depends primarily on the coaxial stacking of staples that are adjacent on the same helix, a parameter that can be modified with staple design. Creating a nucleation barrier to DNA-origami assembly could be useful in optimizing assembly times and yields, while eliminating the barrier may allow for fast molecular sensors that can assemble/disassemble without hysteresis in response to changes in the environment.

==> tex/macros_arxiv.tex <==
% macros_arxiv.tex

\makeatletter
\newcommand{\defaultcolor}[1]{%
  \color{#1}\global\let\default@color\current@color
}
\makeatother

\newcommand\supplemental{%
    \xdef\presupfigures{\arabic{figure}}% save the current figure number
    \xdef\presupsections{\arabic{section}}% save the current section number
    \xdef\presupequations{\arabic{equation}}% save the current section number
    \renewcommand\thefigure{S\fpeval{\arabic{figure}-\presupfigures}}
    \renewcommand\thesection{S\fpeval{\arabic{section}-\presupsections}}
    \renewcommand\theequation{S\fpeval{\arabic{equation}-\presupequations}}
}

% Redefine \maketitle so that it can be used twice (for supplementary)
\makeatletter
\def\maketitle{
\@author@finish
\title@column\titleblock@produce
\suppressfloats[t]}
\makeatother

% horrible stuff for pdflatex
\DeclareUnicodeCharacter{2009}{\,}

% Unit vector
\newcommand{\uvec}[1]{\hat#1}

% Boltzmann constant
\newcommand{\kb}{k_{\mathrm{B}}}

% Avogadro's number
\newcommand{\an}{N_{\mathrm{A}}}

% Standard Gibbs
\newcommand{\dgs}{\upDelta G^{\standardstate}}

% Standard NN Gibbs
\newcommand{\dgsnn}{\upDelta G^{\standardstate}_{\mathrm{NN}}}

% Standard NN enthalpy
\newcommand{\dhsnn}{\upDelta H^{\standardstate}_{\mathrm{NN}}}

% Standard NN entropy
\newcommand{\dssnn}{\upDelta S^{\standardstate}_{\mathrm{NN}}}

% Gibbs intiation
\newcommand{\dgsi}{\dgs_{\textrm{init}}}

% Gibbs symmetry
\newcommand{\dgss}{\dgs_{\textrm{sym}}}

% Gibbs stack
\newcommand{\dgsst}{\dgs_{\textrm{stack}}}

% Gibbs AT terminal
\newcommand{\dgsat}{\dgs_{\textrm{term}}}

% Comments by DF
%\newcommand{\DFcomment}[1]{\todo[inline,size=\normalsize]{[DF]:~#1}}

% Comments by AR
%\newcommand{\ARcomment}[1]{\todo[inline,size=\normalsize,color=blue!20]{[AR]:~#1}}

% Comments by AMC
%\newcommand{\AMCcomment}[1]{\todo[inline,size=\normalsize,color=green!20]{[AMC]:~#1}}

% Units
\DeclareSIUnit\Molar{M}
\DeclareSIUnit\kBT{\ensuremath{\mathit{\kb T}}}
\DeclareSIUnit\kB{\ensuremath{\mathit{\kb}}}

\endinput

